Open Charm Mesons at the LHC with ALICE

The ALICE experiment will be able to detect hadrons containing charm and beauty quarks in proton-proton and heavy ion collisions in the new energy regime of the CERN Large Hadron Collider (LHC). Open charmed mesons are a powerful tool to study the medium produced in heavy ion collisions, since charm quarks are produced on a very short time scale and they experience the whole history of the collision. In addition, the measurements of heavy flavour yield provide a natural normalization for those of charmonia and bottomonia production at LHC. In this talk, after a general overview of ALICE perspectives for heavy flavour physics, we will report some study of D-meson reconstruction through their hadronic decay channels with Monte Carlo simulated data.

==> README <==
This is the README file for camera.cls and template.tex
-----------------------------------------------------------------

This package is in ftp://ftp.sif.it/pub/tex/camera-ready/

camera is a LaTeX mini-package for preparing camera-ready papers
to be published by the Societ\`a Italiana di Fisica.

camera.cls:    LaTeX2e version. Take this one if you have LaTeX2e
template.tex:  A paper template.


The latex 2.09 version camera.sty is no longer supported and has been
removed.

----------------------------------------------------------
For any question, write to marco@sif.it
See also http://www.sif.it

